It's Not a Modality Gap: Characterizing and Addressing the Contrastive Gap

Multi-modal contrastive models such as CLIP achieve state-of-the-art performance in zero-shot classification by embedding input images and texts on a joint representational space. Recently, a modality gap has been reported in two-encoder contrastive models like CLIP, meaning that the image and text embeddings reside in disjoint areas of the latent space. Previous studies suggest that this gap exists due to 1) the cone effect, 2) mismatched pairs in the dataset, and 3) insufficient training. We show that, even when accounting for all these factors, and even when using the same modality, the contrastive loss actually creates a gap during training. As a result, We propose that the modality gap is inherent to the two-encoder contrastive loss and rename it the contrastive gap. We present evidence that attributes this contrastive gap to low uniformity in CLIP space, resulting in embeddings that occupy only a small portion of the latent space. To close the gap, we adapt the uniformity and alignment properties of unimodal contrastive loss to the multi-modal setting and show that simply adding these terms to the CLIP loss distributes the embeddings more uniformly in the representational space, closing the gap. In our experiments, we show that the modified representational space achieves better performance than default CLIP loss in downstream tasks such as zero-shot image classification and multi-modal arithmetic.

==> 1.abstract.tex <==
% NOT USING THIS FILE ANYMORE


Multimodal contrastive models such as CLIP (\cite{clip}) achieve state-of-the-art performance in zero-shot classification by embedding input images and texts on a joint representational space. Recently a  \emph{modality gap} has been reported in two-encoder contrastive models like CLIP, meaning that the image and text embeddings reside in disjoint areas of the latent space. Previous studies suggest that this gap exists due to 1) the cone effect, 2) mismatched pairs in the dataset, and 3) insufficient training. We show that, even when accounting for all these factors, and even when using the \emph{same modality}, the contrastive loss actually \emph{creates} a gap during training. We present evidence that attributes this modality gap to low uniformity in the high-dimensional CLIP space, resulting in embeddings that occupy only a small portion of the latent space.  We then show that modifying the CLIP loss to include explicit uniformity and alignment terms distributes the embeddings more uniformly in CLIP space, closing the gap. In our experiments, we show that the modified representational space achieves better performance in downstream tasks such as zero-shot image classification and multi-modal arithmetic. We propose that the modality gap is inherent to the two-encoder contrastive loss and rename it the \emph{contrastive gap}. 

% We then show that modifying the CLIP loss to include explicit uniformity and alignment terms distributes the embeddings more uniformly in CLIP space, closing the gap. This better-distributed embedding space improves the alignment of image-text pairs, positively impacting downstream task performance. We propose that the modality gap is inherent to the two-encoder contrastive loss and rename it the \emph{contrastive gap}. 

% We present evidence that attributes this modality gap to differences in the rank of the input and the dimensionality of the learned CLIP space, resulting in embeddings that occupy only a small portion of CLIP space. We propose that the modality gap is inherent to multimodal contrastive loss and rename it the \emph{contrastive gap}. 


% VER 5
% Multimodal contrastive models such as CLIP (\cite{clip}) achieve state-of-the-art performance in zero-shot classification by embedding input images and texts on a joint representational space. Recently a  \emph{modality gap} has been reported in two-encoder contrastive models like CLIP, meaning that the image and text embeddings reside in disjoint areas of the latent space. Previous studies suggest that this gap exists due to 1) the cone effect, 2) mismatched pairs in the dataset, and 3) insufficient training. We show that, even when accounting for all these factors, the gap still persists. We present evidence that attributes the modality gap to differences in the rank of the input and the dimensionality of the learned CLIP space, resulting in embeddings that occupy only a small portion of CLIP space.

% VER 4
% We show that modifying the CLIP loss to include separate uniformity and alignment terms distributes the embeddings more uniformly throughout the CLIP space, closing the modality gap. This better-distributed embedding space aligns positive image-text pairs more strongly, positively impacting downstream task performance. 

% Our experiments show that our new loss reduces the modality gap, while increasing performance metrics such as zero-shot image classification accuracies and linear probe accuracies on standard image classification benchmarks. This work provides a proof-of-concept for increasing the quality of CLIP representations through closing the modality gap.

% VER 3
% We propose that distributing the CLIP embeddings in a higher dimensional manifold would close the modality gap. To that end, we modify the CLIP loss to include separate uniformity and alignment terms, which distributes the embeddings more uniformly throughout the CLIP space, while aligning positive image-text pairs more strongly. Our experiments show that our new loss reduces the modality gap, while increasing performance metrics such as zero-shot image classification accuracies and linear probe accuracies on standard image classification benchmarks. This work provides a proof-of-concept for increasing the quality of CLIP representations through closing the modality gap.

% VER 2
% The modality gap is a phenomenon observed in two-encoder contrastive learning algorithms such as CLIP ~\cite{clip}. CLIP learns to embed input images and texts on a joint representation space. As the name Modality Gap suggests, there is a "gap" between the output embeddings of the image and text encoders of CLIP. Previous work has suggested that this gap exists due to 1) the cone effect, 2) mismatched pairs in the datset, 3) insufficient training, and 4) information gap between modalities. In this paper we show that, even when accounting for all these factors, the gap still persists. We then reason about the modality gap in terms of the dimensionality of the learned CLIP space. We show that the modality gap is a symptom of CLIP embeddings lying on a lower dimensional manifold relative to the dimensionality of the CLIP latent space. This results in CLIP embeddings occupying only a small portion of the unit hypersphere. 


% The modality gap is a phenomenon observed in two-encoder contrastive learning algorithms such as CLIP ~\cite{clip}. CLIP learns to embed input images and texts on a joint representation space. As the name Modality Gap suggests, there is a "gap" between the output embeddings of the image and text encoders of CLIP. Previous work has suggested that this gap exists due to 1) the cone effect, 2) mismatched pairs in the datset, 3) insufficient training, and 4) information gap between modalities. In this paper we show that, even when accounting for all these factors, the gap still persists. We then reason about the modality gap in terms of the dimensionality of the learned CLIP space. We show that the modality gap is a symptom of CLIP embeddings lying on a lower dimensional manifold relative to the dimensionality of the CLIP latent space. This results in CLIP embeddings occupying only a small portion of the unit hypersphere. 


% VER 1
% The modality gap is a phenomenon recently brought to light in two-encoder contrastive learning algorithms (such as CLIP ~\cite{}, which is trained on two modalities (images and texts)). As the name suggests, there is a "gap" between the output embeddings of the two encoders. Previous work has suggested that this gap exists due to 1) the cone effect, 2) mismatched pairs in the datset, 3) insufficient training, and 4) information gap between modalities. In this paper we show that, even when accounting for all these factors, the gap still persists. We then reason about the modality gap in terms of the dimensionality of the learned CLIP space. We show that the modality gap arises when CLIP space is too high dimensional relative to batch size, allowing CLIP embeddings to occupy only a small portion of the unit hypersphere. 

% To close the modality gap, and to encourage CLIP embeddings to occupy more of the unit hypersphere, we modify the CLIP loss to include a uniformity term, which distributes the embeddings more uniformly throughout the CLIP space. Our preliminary experiments show a <percentage improvement> improvement in zero shot image classification tasks over default CLIP. 

\endinput

==> ack.tex <==
%\section{Acknowledgment}
\textbf{Acknowledgments:} Later

